A Collaborative Filtering Recommender System for Test Case Prioritization in Web Applications

The use of relevant metrics of software systems could improve various software engineering tasks, but identifying relationships among metrics is not simple and can be very time consuming. Recommender systems can help with this decision-making process, many applications have utilized these systems to improve the performance of their applications. To investigate the potential benefits of recommender systems in regression testing, we implemented an item-based collaborative filtering recommender system that uses user interaction data and application change history information to develop a test case prioritization technique. To evaluate our approach, we performed an empirical study using three web applications with multiple versions and compared four control techniques. Our results indicate that our recommender system can help improve the effectiveness of test prioritization.

==> abstract.tex <==
\begin{abstract}
The use of relevant metrics of software systems could improve
various software engineering tasks, but identifying relationships among
metrics is not simple and can be very time consuming. 
Recommender systems can help with this decision-making process; many applications
have utilized these systems to improve the performance of their applications.
To investigate the potential benefits of recommender systems in regression 
testing, we implemented an item-based collaborative filtering recommender
system that uses user interaction data and application change history 
information to develop a test case prioritization technique.
To evaluate our approach, we performed an empirical study using three 
applications with multiple versions and compared five control techniques.
Our results indicate that our recommender system can help improve the 
effectiveness of test prioritization; the performance of our approach
was particularly  noteworthy when we were under a time constraint.  
\end{abstract}



==> algorithm.tex <==
\begin{algorithm}[!b]
\vspace*{3pt}
%\begin{algorithm}[ht]
\caption{Path Generation}\label{fig:pathAlgol}
\begin{algorithmic}[1]
{\footnotesize
\State \textbf{Inputs:} \textbf{ \textit{slices[]}} \Comment{\textit{The slices
array contains all of the slices
that are generated by the analyzing changes made to the modified version of the application.}}
\State \textbf{Outputs:} \textbf{\textit{paths}} \Comment{\textit{An array of all of the linearly
independent paths produced from the set of slices.}} 
\State \textbf{Declare:} \textbf{\textit{edges}} \Comment{\textit{A set of edges traveled by the path 
generator}}
\State \textbf{\textit{currentPath}} \Comment {\textit{A placeholder for the path currently being
generator}}
\Procedure{PathGeneration}{$slices$}
	\State $paths \gets \emptyset$ 
	\State $edges \gets \emptyset$ 
	\For{$n \longleftarrow 0 $, $n < slices$.size(), $n$++}
	\While{$slices[n]$.size()$ > 0$}
		\State $currentNode \gets slice[n]$.firstNode()
	    \State $currentPath \gets \emptyset$ 
	    \State $currentPath$.add($currentNode$)
	    \State PDGTraverser($currentPath$, $paths$, $edges$, $slice[n]$, $currentNode$) 
	\EndWhile\label{mainPathWhile}
	\EndFor
	\State ResolvePaths();
	\State \textbf{return} $paths$
	\EndProcedure
}
\end{algorithmic}
\end{algorithm}


==> ast.tex <==

\subsection{Preprocessing}
\label{sec:preprocess}

%Before we performed the impact analysis on two consecutive 
%versions of PHP web applications, we performed 
%two preprocessing steps to address the challenges associated 
%with analyzing a high-level, dynamic programming language. 
%The following subsections describe each step in detail.
%
%\subsubsection{File Preparation}
%\label{sec:fileprep}
%
%PARTE uses abstract syntax trees (ASTs) to generate PDGs.
%To create ASTs from PHP programs, we used PHC (a PHP compiler),
%which is a publicly available, open source tool.
%We used PHC because it generates the ASTs that contain detailed 
%information about variable data types that is necessary for input 
%data constraint gathering and resolution. 
%
%However, there are a couple problems with PHC. 
%PHC cannot properly parse \textit{include} and \textit{require} 
%functions that contain variables instead of constant strings. 
%Futher, PHC cannot properly evaluate the expressions if any 
%concatenation or defined values are used in the \textit{include} 
%or \textit{require} function.
%Using defined values and runtime concatenation 
%to include a specified file in a location defined during the 
%installation of the web application is a common practice.
%
%Since PHC cannot resolve non-trivial \textit{include} and 
%\textit{require} function calls, we built a parsing tool that searches 
%for them through the web application source code and then locates, 
%defines, and stores them in a dictionary. When the parsing tool locates 
%\textit{include} or \textit{require} function names, it resolves 
%them using the dictionary that maintains defined values. 
%If \textit{include} or \textit{require} functions are completely 
%resolved, the tool inserts their code into the associated 
%source code. This process is repeated until the tool 
%visits every \textit{include} and \textit{require} function.
%
%Another common feature of many dynamic web applications is to specify 
%which files to include at runtime. One typical example of this feature 
%is that a user selects a language preference when the web application 
%is presented. For cases like this one, we manually assign a 
%constant value to the environmental variable in the application. 
%
%\subsubsection{AST2HIR}
%\label{sec:ast2hir}
%
%After we obtained the preprocessed PHP files from the previous step,    
%we generate ASTs for these PHP files using PHC.
%Then, we covert AST to a high-level intermediate representation (HIR) 
%to simplify PDG generation. PHC already provides a function that 
%generates HIR code from an AST, but the HIR code generated by PHC does 
%not preserve consistent variable names across versions of the same 
%application, so it is not suitable for our regression testing tasks. 
%PHC's HIR is focused on code optimization for performance efficiency.
%
%PHC uses a typical three-address code generation approach and creates 
%variable names by incrementing a numerical suffix on a fixed prefix. 
%Thus, if a single statement in a program is added, deleted, 
%or modified, every statement that comes after it in the internal 
%representation could have variable names that do not correspond with 
%the variable names in the original version's internal representation. 
%Our regression testing framework requires consistent variable names 
%to properly generate an impact set given two different versions of 
%the PHP program.
%To resolve this issue, we implemented an AST2HIR tool that maintains 
%consistent variable names while generating a three-address 
%code representation of the program. Instead of simply incrementing 
%based on the order variables appeared in a source file, we used 
%a hashing function on the values from the control dependency 
%information combined with the expression values within a statement 
%from the AST to determine variable names.
%
%There are two main types of symbols in the AST: statements and 
%expressions. Statements are the symbols that define classes, interfaces, 
%and methods as well as the control flow of the program. Expressions 
%are the rest of the symbols, some of which include arithmetic operators, 
%conditional expressions, assignments, method invocations, and logical 
%operators. The AST that PHC generates is in XML format, and the AST2HIR 
%converter parses the XML tags in a depth-first manner. 
%%There is a difference between the parsing method of statements and 
%%expressions. Statements are parsed before their child nodes are parsed 
%%while expressions are only parsed after their child nodes.
%When a complex statement (``complex'' being defined as an expression 
%that is not in formatted, three-address code) is encountered while 
%parsing, it is split into multiple expressions such that all parts 
%are not complex. These parts are given a unique variable name, 
%and assignment expressions are generated to assign the value of 
%the non-complex parts to their corresponding unique variables.
%Some statements are also transformed to work in the PDG generator. 
%For instance, a ``for'' loop is simplified into a ``while'' loop. 
%``Switch'' statements are converted into equivalent code using a 
%``while'' loop, ``if'' statements, and ``break'' statements.
%
%The AST2HIR tool then produces a PHP program that is functionally 
%equivalent to the original program but in the high-level internal 
%representation. An AST for this HIR program is then created using 
%PHC. This HIR version of the AST is used to generate the PDGs. 
%Throughout the paper, we refer to this HIR version of the AST
%simply as AST.
%


==> impact.tex <==

\subsection{Impact Analysis}

%To analyze the impact of software modifications on a web
%application, we implemented a static program slicer for web
%applications written in the PHP programming language. 
%The benefit of using a program slicer is that it provides 
%a complete way to reveal which areas of the application will 
%be affected by software modifications~\cite{agrawal90}.
%
%Using the ASTs we constructed during the preprocessing steps, 
%we perform the impact analysis that identifies the areas of 
%the application that have been affected by code changes. 
%For impact analysis, three steps are involved: PDG generation,
%program differencing, and program slicing. 
%
%To build PDGs from ASTs, we follow the same approach
%used by Harrold et al.~\cite{harrold93}. 
%First, the PDG generator constructs control flow graphs. 
%During this phase, the PDG generator builds control flow graphs 
%for all methods and functions that have been declared. 
%To construct an inter-procedural control flow graph, all method 
%or function calls within the control flow graphs are linked to 
%their corresponding control flow graphs.
%Next, the PDG generator analyzes the data by performing a def-use 
%analysis, and it gathers data dependency information for variables. 
%%The PDG generator uses a bit-vector to track the 
%%definitions and uses of variables throughout the application. 
%
%After constructing PDGs for two consecutive versions,
%we need to determine which files have been changed from the
%previous version and which statements within these files have
% been changed. To perform this task, we use a textual differencing 
%approach similar to that of the standard Unix diff tool. In our 
%approach, the differencing tool compares two versions of program 
%dependence graphs, in XML format, that contain the program structure 
%and statement content. The differencing tool analyzes each program 
%and applies a longest common subsequence approach on the PDG 
%representation of the statements.
%After the tool determines which statements have been edited, added, 
%or deleted, it provides this information to the program slicer.
%
%Finally, the program slicer creates program slices by using
%the program modification information. Program slicing is a technique 
%that can be used to trace control and data dependencies with 
%an application~\cite{weiser81}, and in this work, it is used for 
%calculating the code change impact set. Our program slicer performs 
%forward slicing by finding all statements that are data dependent on 
%the variables defined in the modified statements and produces a program 
%slice following these dependencies. It then performs backward slicing 
%on the modified statements to determine the statements upon which each 
%modified statement is data dependant. For each modified statement, 
%the forward and backward slices are combined into a single slice.


